GUIOpsBench: Evaluating Multimodal Agents on GUI-Centric Cloud Operations

Routine cloud administration requires operators to interpret visual dashboards, navigate dense interfaces, and follow procedural instructions across multiple console pages. These workflows are not directly assessed by telemetry-centered AIOps benchmarks or general-purpose GUI-agent benchmarks. Motivated by an industrial study of routine operations, we introduce GUIOpsBench, a benchmark for evaluating vision-language models on cloud management consoles. GUIOpsBench contains 21,680 annotated samples from AWS, Google Cloud, Alibaba Cloud, and Volcengine, organized into Ops-UI Understanding, Ops-Action Grounding, and Ops-Task Completion. A dual-path collection engine combines SOP-guided trajectory generation with exploration-driven semantic reconstruction to capture both documented procedures and a broader range of interface states. Evaluations of seven proprietary and open-source models reveal substantial limitations in domain-specific understanding and precise visual interaction. The best average grounding accuracy is 19.09%, and the highest average task success rate using screenshots alone is 13.7%. With DOM-assisted grounding and multi-agent execution in TrajMAS, the highest average task success rate rises to 50.1%, while substantial room for improvement remains. These results identify visual grounding and operational knowledge as key challenges for reliable GUI-based cloud automation.

==> tab/understanding_model.tex <==

% \usepackage{booktabs}
% \usepackage{multirow}

\begin{table}[t]
\centering
\caption{Detailed performance breakdown by model. The highest scores within each task category are marked in bold.}
\label{tab:model_performance_detailed}
\vspace{0.08in}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
\textbf{Model} & \textbf{Task} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} & \textbf{Sim} \\
\midrule
\multirow{5}{*}{CS4.5}
 & DI  & 0.4560 & 0.8059 & 0.5636 & 0.8795 \\
 & NAV & 0.5028 & 0.8869 & 0.6117 & 0.9002 \\
 & PO  & 0.3159 & 0.7804 & 0.4335 & 0.8342 \\
 & SO  & 0.3422 & \textbf{0.8181} & 0.4688 & 0.8558 \\
 & UI  & 0.4410 & \textbf{0.9012} & 0.5746 & 0.8663 \\
\midrule
\multirow{5}{*}{GPT4o}
 & DI  & \textbf{0.6040} & 0.6588 & 0.6134 & 0.9038 \\
 & NAV & \textbf{0.6856} & 0.8102 & 0.7078 & 0.9239 \\
 & PO  & 0.4420 & 0.6347 & 0.5025 & 0.8554 \\
 & SO  & 0.4478 & 0.6429 & 0.5095 & 0.8702 \\
 & UI  & 0.5979 & 0.7636 & \textbf{0.6533} & 0.8946 \\
\midrule
\multirow{5}{*}{GPT5.2}
 & DI  & 0.5022 & \textbf{0.8381} & 0.6091 & \textbf{0.9160} \\
 & NAV & 0.5950 & \textbf{0.9495} & 0.7055 & \textbf{0.9383} \\
 & PO  & 0.3300 & \textbf{0.8316} & 0.4559 & \textbf{0.8970} \\
 & SO  & 0.3324 & 0.7540 & 0.4480 & \textbf{0.9084} \\
 & UI  & 0.4132 & 0.7829 & 0.5262 & \textbf{0.9035} \\
\midrule
\multirow{5}{*}{G3-F}
 & DI  & 0.4862 & 0.7265 & 0.5644 & 0.8244 \\
 & NAV & 0.5681 & 0.8261 & 0.6399 & 0.8525 \\
 & PO  & 0.3700 & 0.7304 & 0.4729 & 0.8212 \\
 & SO  & 0.3807 & 0.7338 & 0.4859 & 0.8316 \\
 & UI  & 0.4863 & 0.8382 & 0.5996 & 0.8372 \\
\midrule
\multirow{5}{*}{IVL}
 & DI  & 0.5977 & 0.6206 & 0.5909 & 0.8943 \\
 & NAV & 0.6701 & 0.8245 & 0.7134 & 0.9186 \\
 & PO  & \textbf{0.4666} & 0.6738 & \textbf{0.5259} & 0.8467 \\
 & SO  & \textbf{0.4818} & 0.6683 & \textbf{0.5409} & 0.8587 \\
 & UI  & \textbf{0.6085} & 0.7371 & 0.6485 & 0.8794 \\
\midrule
\multirow{5}{*}{Q3-VL}
 & DI  & 0.5571 & 0.7651 & \textbf{0.6235} & 0.9067 \\
 & NAV & 0.5911 & 0.8630 & 0.6664 & 0.9176 \\
 & PO  & 0.3571 & 0.6684 & 0.4482 & 0.8488 \\
 & SO  & 0.3918 & 0.7913 & 0.5083 & 0.8714 \\
 & UI  & 0.4923 & 0.8349 & 0.6018 & 0.8847 \\
\midrule
\multirow{5}{*}{S1.6}
 & DI  & 0.4213 & 0.6054 & 0.4820 & 0.8731 \\
 & NAV & 0.6758 & 0.8535 & \textbf{0.7305} & 0.9117 \\
 & PO  & 0.2778 & 0.5357 & 0.3519 & 0.8261 \\
 & SO  & 0.1566 & 0.2806 & 0.1958 & 0.8404 \\
 & UI  & 0.3473 & 0.5618 & 0.4183 & 0.8538 \\
\bottomrule
\end{tabular}%
}
\vspace{0.05in}

\footnotesize
\textbf{Abbreviations:}
DI = Data Interpretation, NAV = Navigation, PO = Page Overview, SO = Specific Operation, UI = UI Element.
C-S4.5 = Claude-Sonnet-4.5, GPT4o = GPT-4o, GPT5.2 = GPT-5.2, G3-F = Gemini-3-Flash, IVL = InternVL, Q3-VL = Qwen-3-VL, S1.6 = Seed-1.6.
\end{table}


==> tab/understanding_type.tex <==

% \usepackage{booktabs}
% \usepackage{multirow}

\begin{table}[t]
\centering
\caption{Performance comparison of different models across various task types. The best scores in each category are highlighted in bold.}
\label{tab:model_performance}
\vspace{0.08in}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
\textbf{Type} & \textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} & \textbf{Sim} \\
\midrule
\multirow{7}{*}{DI}
 & CS4.5 & 0.4560 & 0.8059 & 0.5636 & 0.8795 \\
 & GPT4o  & \textbf{0.6040} & 0.6588 & 0.6134 & 0.9038 \\
 & GPT5.2 & 0.5022 & \textbf{0.8381} & 0.6091 & \textbf{0.9160} \\
 & G3-F   & 0.4862 & 0.7265 & 0.5644 & 0.8244 \\
 & IVL    & 0.5977 & 0.6206 & 0.5909 & 0.8943 \\
 & Q3-VL  & 0.5571 & 0.7651 & \textbf{0.6235} & 0.9067 \\
 & S1.6   & 0.4213 & 0.6054 & 0.4820 & 0.8731 \\
\midrule
\multirow{7}{*}{NAV}
 & CS4.5 & 0.5028 & 0.8869 & 0.6117 & 0.9002 \\
 & GPT4o  & \textbf{0.6856} & 0.8102 & 0.7078 & 0.9239 \\
 & GPT5.2 & 0.5950 & \textbf{0.9495} & 0.7055 & \textbf{0.9383} \\
 & G3-F   & 0.5681 & 0.8261 & 0.6399 & 0.8525 \\
 & IVL    & 0.6701 & 0.8245 & 0.7134 & 0.9186 \\
 & Q3-VL  & 0.5911 & 0.8630 & 0.6664 & 0.9176 \\
 & S1.6   & 0.6758 & 0.8535 & \textbf{0.7305} & 0.9117 \\
\midrule
\multirow{7}{*}{PO}
 & CS4.5 & 0.3159 & 0.7804 & 0.4335 & 0.8342 \\
 & GPT4o  & 0.4420 & 0.6347 & 0.5025 & 0.8554 \\
 & GPT5.2 & 0.3300 & \textbf{0.8316} & 0.4559 & \textbf{0.8970} \\
 & G3-F   & 0.3700 & 0.7304 & 0.4729 & 0.8212 \\
 & IVL    & \textbf{0.4666} & 0.6738 & \textbf{0.5259} & 0.8467 \\
 & Q3-VL  & 0.3571 & 0.6684 & 0.4482 & 0.8488 \\
 & S1.6   & 0.2778 & 0.5357 & 0.3519 & 0.8261 \\
\midrule
\multirow{7}{*}{SO}
 & CS4.5 & 0.3422 & \textbf{0.8181} & 0.4688 & 0.8558 \\
 & GPT4o  & 0.4478 & 0.6429 & 0.5095 & 0.8702 \\
 & GPT5.2 & 0.3324 & 0.7540 & 0.4480 & \textbf{0.9084} \\
 & G3-F   & 0.3807 & 0.7338 & 0.4859 & 0.8316 \\
 & IVL    & \textbf{0.4818} & 0.6683 & \textbf{0.5409} & 0.8587 \\
 & Q3-VL  & 0.3918 & 0.7913 & 0.5083 & 0.8714 \\
 & S1.6   & 0.1566 & 0.2806 & 0.1958 & 0.8404 \\
\midrule
\multirow{7}{*}{UI}
 & CS4.5 & 0.4410 & \textbf{0.9012} & 0.5746 & 0.8663 \\
 & GPT4o  & 0.5979 & 0.7636 & \textbf{0.6533} & 0.8946 \\
 & GPT5.2 & 0.4132 & 0.7829 & 0.5262 & \textbf{0.9035} \\
 & G3-F   & 0.4863 & 0.8382 & 0.5996 & 0.8372 \\
 & IVL    & \textbf{0.6085} & 0.7371 & 0.6485 & 0.8794 \\
 & Q3-VL  & 0.4923 & 0.8349 & 0.6018 & 0.8847 \\
 & S1.6   & 0.3473 & 0.5618 & 0.4183 & 0.8538 \\
\bottomrule
\end{tabular}%
}
\vspace{0.05in}

\footnotesize
\textbf{Abbreviations:}
DI = Data Interpretation, NAV = Navigation, PO = Page Overview, SO = Specific Operation, UI = UI Element.
C-S4.5 = Claude-Sonnet-4.5, GPT4o = GPT-4o, GPT5.2 = GPT-5.2, G3-F = Gemini-3-Flash, IVL = InternVL, Q3-VL = Qwen-3-VL, S1.6 = Seed-1.6.
\end{table}

